Towards More Equitable Question Answering Systems: How Much More Data Do You Need?

Question answering (QA) in English has been widely explored, but multilingual datasets are relatively new, with several methods attempting to bridge the gap between high- and low-resourced languages using data augmentation through translation and cross-lingual transfer. In this project, we take a step back and study which approaches allow us to take the most advantage of existing resources in order to produce QA systems in many languages. Specifically, we perform extensive analysis to measure the efficacy of few-shot approaches augmented with automatic translations and permutations of context-question-answer pairs. In addition, we make suggestions for future dataset development efforts that make better use of a fixed annotation budget, with a goal of increasing the language coverage of QA datasets and systems. Code and data for reproducing our experiments are available here: https://github.com/NavidRajabi/EMQA.

==> A3.tex <==
\section{Baseline Problem Description}
\label{section:BaselineProblemDescription}
%In this milestone of the project (Assignment 3), we've tried to reproduce the baseline results of the Gold Passage task \cite{Github:NLP-Assignment-3} of the TyDi QA benchmark \cite{clark2020tydi}. 


\subsection{Gold-Passage Task}
The Gold Passage task of TyDi QA benchmark \cite{clark2020tydi} consists of two major parts: (1) Training and evaluation on TyDi QA, and (2) Training on SQUAD, but evaluation on TyDi QA (so called Zero-Shot SQUAD). To be more specific, the structure of the TyDiQA/SQUAD are as follows.
Each instance of the dataset consists of 5 key-pair values: (1) "id" , (2) "title", (3) "context", (4) "question" , and (5) "answers". 
In the Gold passage task, the passage that is guaranteed to include the answer for the proposed question is given, instead of the full document. Consequently, given the Gold Passage, the output result would be the minimal span of the predicted answer, similar to the other question answering tasks.
The major reason why we picked the Gold passage task is the compatibility with the previous well-known datasets (like SQuAD \cite{rajpurkar2016squad}, XQuAD  \cite{artetxe2020crosslingual}, and MLQA  \cite{lewis2019mlqa}). In this way, there would be more room for improvement in the next milestone since we would be able to leverage more data from the same structure to pre-train/fine-tune to increase the performance of the baselines on TyDi QA validation set. On the other hand, any performance improvement on TyDi QA can be applied to the other benchmarks as well. 

%Arabic	%Bengali	%Finnish	%Indonesian	%Kiswahili	%Russian	%Telugu

\begin{table*}[h]
%   \caption{Experiment Definitions Overview} \label{table:experimentDefinitions}
  \centering
  \begin{tabular}{llllr}
    \toprule
    Task ID                    & Pre-trained  & Fine-tuned      &  Evaluated      & Results  \\ \midrule
    \multirow{1}{*}{Zero-shot}   &  SQuAD       &  -              &  TyDi QA       &    \\
                               &  Train Set   &                 &  Dev Set       &  \\ \addlinespace
    \multirow{1}{*}{Baseline}   &  TyDi QA       &  -              &  TyDi QA       &    \\
            Re-production      &  Train Set   &                 &  Dev Set       &  \\ \addlinespace
    % \multirow{1}{*}{Task 0B}   &  SQuAD       & Few TyDi QA     &  TyDi QA       &    \\
    %                           &  Train Set   & train instances &  Dev Set       &  \\ \addlinespace
    \multirow{1}{*}{Task 1}    &  SQuAD Train Set       &  -       &  TyDi QA  \\
                               &  + All SQuAD translations   &    &  Dev Set        &  \\ \addlinespace
    \multirow{1}{*}{Task 2}   &  SQuAD       & Few QA pairs from &  TyDi QA     &    \\
                               &  Train Set   & translated SQuAD &   Dev Set     &  \\ \addlinespace
    \multirow{1}{*}{Task 3A}   &  SQuAD       & Few unique QA pairs & TyDi QA    &    \\
                               &  Train Set   & from translated SQuAD &  Dev Set       &  \\ \addlinespace
    \multirow{1}{*}{Task 3B}   &  SQuAD       & Few TyDi QA     &   TyDi QA             &    \\
                               &  Train Set   & train instances &   Dev Set             &  \\ \addlinespace
    \multirow{1}{*}{Task 3C}   &  SQuAD Train Set      & 500 TyDi QA  &  TyDi QA            &    \\
                               &  + All SQuAD translations   & train instances &  Dev Set &  \\ \addlinespace
    \multirow{1}{*}{Task 3C-1} &  SQuAD Train Set      &   Disproportional TyDi QA    &  TyDi QA              &    \\
                               &  + All SQuAD translations   &   allocation (all languages)          & Dev Set                &  \\ \addlinespace
    \multirow{1}{*}{Task 3C-2} &  SQuAD Train Set      &   Disproportional TyDiQA    &  TyDi QA              &    \\
                               &  + All SQuAD translations   &   allocation (random 3 languages)    &  Dev Set               &  \\ \addlinespace
    \multirow{1}{*}{Task 4A}   &  Modified SQuAD &        -      &     TyDi QA           &    \\
                               &  C-A: English; Q: Random   &   &     Dev Set           &  \\ \addlinespace
    \multirow{1}{*}{Task 4B}   &  Modified SQuAD        &    -  &    TyDi QA        &    \\
                               &  C-A: Random; Q: Random        &   &   Dev Set             &  \\ \addlinespace
    \multirow{1}{*}{Task 5}    &  SQuAD Train Set  &  All XQuAD translations  &       TyDi QA       &    \\
                               &  + All SQuAD translations   &  + 500 TyDi QA train   &    Dev Set     &  \\ \bottomrule
    % Task 5                   &      &       \\ \bottomrule
  \end{tabular}
  \caption{Experiment Definitions Overview} \label{table:experimentDefinitions}
\end{table*}



% \begin{figure}[h!]
% \centering
% \scalebox{0.8}{
% \includegraphics[width =0.56\textwidth,, frame]{Figures/tydiqa_tydiqa.png}}
% \caption{TYDIQA-GOLDP task v1.1  F1  scores against Epochs : pre-trained on mBERT, fine tuned on TYDIQA-GOLDP train v1.1 dataset and evaluated on TYDIQA-GOLDP dev set}
% \label{fig:tydiqa_tydiqa_graph}
% \end{figure}

\begin{figure}[h]
\centering
\includegraphics[scale=0.55, center]{Figures/mBERT-TyDiQA-HQ-Serif.jpg}
\caption{Full TyDi QA Gold-Passage Baseline Reproduction Results vs. Number of Epochs}
\label{fig:tydiqa_tydiqa_graph}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[scale=0.55, center]{Figures/SQUAD-Zeroshot-TyDiQA-HQ-Serif.jpg}
\caption{SQuAD Zero-shot on TyDi QA Baseline Reproduction Results vs. Number of Epochs}
\label{fig:squad_tydiqa_graph}
\end{figure}

% \vspace{3mm}
% \begin{figure}[h!]
% \centering
% \scalebox{0.8}{
% \includegraphics[width =0.56\textwidth,, frame]{Figures/squad_tydiqa.png}}
% \caption{TYDIQA-GOLDP task v1.1  F1  scores against Epochs : pre-trained on mBERT, fine tuned on SQuAD v1.1 dataset and evaluated on TYDIQA-GOLDP dev set}
% \label{fig:squad_tydiqa_graph}
% \end{figure}

\subsection{Baseline Results}

\begin{table*}[!ht]
% \caption{TyDi QA Reproduced Results} \label{table:GoldTaskResult}
\centering  % not needed, since table is as wide as text block
\begin{tabularx}{\textwidth}{@{}lYYYY@{}}
\toprule
&\multicolumn{2}{c}{\bfseries TyDi QA Gold Passage}
&\multicolumn{2}{c}{\bfseries SQuAD Zero Shot} \\
\cmidrule(lr){2-3} \cmidrule(l){4-5} 
&Reproduced (Ours)
&Baseline\cite{clark2020tydi}
&Reproduced (Ours)
&Baseline\cite{clark2020tydi} \\
\midrule
English & \textbf{77.51} & 76.8 & \textbf{74.21} & 73.4  \\
Arabic & \textbf{82.44} & 81.7  & 59.01 & \textbf{60.3} \\
Bengali & \textbf{78.94} & 75.4 & 57.25 & \textbf{57.3} \\
Finnish & \textbf{80.06} & 79.4 & 55.67 & \textbf{56.2} \\
Indonesian & \textbf{85.36} & 84.8  & \textbf{63.20} & 60.8 \\
Kiswahili & \textbf{83.78} & 81.9  &  \textbf{60.34} & 52.9  \\
Korean  & 34.55 & \textbf{69.2} & 22.49 & \textbf{50.0}  \\
Russian & \textbf{76.46} & 76.2  & \textbf{65.59} & 64.4  \\
Telugu & 78.27 & \textbf{83.3} & 44.64 & \textbf{49.3}  \\
Overall & 80.76 & \textbf{79.0} & \textbf{57.50} & 56.4  \\
\bottomrule
\end{tabularx}
\caption{TyDi QA Reproduced Results} \label{table:GoldTaskResult}
\end{table*}

% %[Gold-Passage reproduced table results]
% \begin{table}[h]
% \begin{center}
% \centering
% \scalebox{0.78}{
% \begin{tabular}{  |p{1.7cm}||m{2.9cm}|m{2.9cm}|  }\hline
%  \multicolumn{3}{|c|}{F1 scores for the simplified TYDIQA - GOLDP task \newline} \\
%  \hline
%  \hline
% \textbf{Languages} & \textbf{TYDIQA GOLDP/ \#} & \textbf{SQuAD Zero Shot/ \#}\\
%  \hline
% (English)   & \textbf{(77.51)} / (76.8)     & \textbf{(74.21)} / (73.4)\\
%   \hline
% Arabic &   \textbf{82.44} / 81.7   & \textbf{59.01} / 60.3\\
% Bengali & \textbf{78.94} / 75.4 & \textbf{57.25} / 57.3\\
% Finnish   & \textbf{80.06} / 79.4 & \textbf{55.67} / 56.2\\
%   \hline
% Indonesian & \textbf{85.36} / 84.8  & \textbf{63.20} / 60.8\\
% Kiswahili & \textbf{83.78} / 81.9  &  \textbf{60.34} / 52.9 \\
% Korean & \textbf{34.55} / 69.2 & \textbf{22.49} / 50.0\\
%   \hline
% Russian & \textbf{76.46} / 76.2  & \textbf{65.59} / 64.4\\
% Telugu & \textbf{78.27} / 83.3 & \textbf{44.64} / 49.3 \\

%   \hline
% \textbf{OVERALL} & \textbf{77.872} / 79.0 & \textbf{57.50} / 56.4 \\
%  \hline
% \end{tabular}}
% \end{center}
% \caption{F1 scores for the simplified TYDIQA-GOLDP
% task v1.1. Left: Fine tuned and evaluated on the
% TYDIQA-GOLDP set. "\#" indicates the ground truth - result produced by Table 7 in \cite{clark2020tydi}. Right: Fine tuned on SQuAD
% v1.1 and evaluated on the TYDIQA-GOLDP dev set. "\#"  indicates the ground truth - result produced by Table 7 in \cite{clark2020tydi}}
% \label{table:GoldTaskResult}
% \end{table}

In Table~\ref{table:GoldTaskResult}, the results of two experiments has been shown for Gold Passage task. First, we
did fine tuning on mBERT based on all the languages of the
TyDi QA gold passage training data and evaluate on its dev set.  For the zero shot experiments, we fine tune on the 100k English-only SQuAD 1.1 training set and evaluate on the TyDi QA gold passage dev set. The result shows our F1 scores are close to the the baseline F1 scores provided in Table 7 in \cite{clark2020tydi}. But the F1 score for Korean languages still remain low which leaves a headroom for future improvement. If we observe the performance of English language, it is significantly lower, demonstrating that the style of question-answer pairs in SQuAD have very limited value in training a model for TyDi QA-style questions, despite the much larger volume of English questions in SQuAD.
 

%\subsection{Conclusion_and_Future_Works}
%To sum up, we've achieved almost the similar performance of mBERT on TyDi QA Gold Passage task compared to the official results mentioned on TyDi QA paper, although with some marginal differences in some languages (except the Korean langauge) as shown in Table \ref{table:GoldTaskResult}. In order to proceed to the next milestone (Assignment 4), we are planning to start with (1) integrating/fine-tuning other pre-trained models (like distil-mBERT \cite{huggingface:distilbert}, XLM \cite{huggingface:xlm}, XLM-RoBERTA  \cite{huggingface:xlmroberta}, and XLM-RoBERTA-Large \cite{huggingface:xlm-roberta-large}), as well as (2) taking advantage of more available multi-lingual question answering benchmarks (like XQuAD and MLQA) to boost the performance of TyDi QA Gold passage for each individual languages and the overall performance. The rational behind choosing this direction is to overcome the issue of data scarcity for the low-resources languages, by incorporating the most powerful pre-trained, multi-lingual language modeling transformers.


==> A4.tex <==
\section{Improvements over the Baselines}
\label{section:ImprovementsovertheBaselines}
In order to improve the baseline performances in Gold-Passage task, we had to either: (1) follow the transfer learning approaches to intensify the performance of existing language models by utilizing a small portion of the TyDi QA training set or (2) focus on improving the full training/testing setting merely based on TyDi QA dataset. Therefore, we formulated the first (transfer learning) approach as "Hypothesis 1" and introduced it as Few-shot setting. Not only this approach is more compliant with the direction of introducing data-efficient models, it was also a novel setting which has not been explored by the TyDi QA benchmark yet. We have mentioned the details and nuances of Hypothesis 1 in section 6.1.  

Moreover, for the second option we had to either replace the current baseline language model (multilingual-BERT) with other pre-trained options, like XLM, XLM-Roberta or XLM-Roberta-Large as one possibility. However, we got slightly lower performance in overall by replacing mBERT with XLMR-Large (which was the most powerful alternative in theory) and did the rest of the experiments using mBERT. Also, we followed another idea in full TyDi QA setting by assuming that the model's perception of different languages is independent, which was different to the way we looked at while reproducing the baseline results. Therefore, we formulated it as ``Hypothesis 2 - Monolingual Full TyDi QA Setting" and explained the details of it's experiments in section 6.2.

% \subsection{Experimental Settings}
% The goal of this section is to detail the experimental settings involved in the improvement of results on the baseline settings.

\subsection{Hypothesis 1 - Few-shot Setting}

Our hypothesis considers that augmenting SQuAD dataset with minimum data for low-resource languages will increase the performance. As a train set, we considered combination of both SQuAD dataset and few instances from TyDi QA train set (monolingual and multilingual settings). And evaluation is performed on the TyDi QA dev set.

Here, instead of taking a percentage of instances from TyDi QA to augment the SQuAD dataset, we have added a fixed number (10, 20 or 50) of random instances, as the TyDi QA dataset is larger than the SQuAD dataset by a good margin. SQuAD dataset has a total of 442 instances while Table \ref{table:TydiQA_no_of_instances} shows the number of instances TyDi QA dataset has for each of the 9 languages.

% \begin{table}[H]
% \centering
% \resizebox{0.35\textwidth}{!}{%
% \begin{tabular}{|l|l|}
% \hline
% TyDiQA Languages & No of instances \\ \hline
% Arabic           & 14805           \\ \hline
% Bengali          & 2390            \\ \hline
% English          & 3696            \\ \hline
% Finnish          & 6855            \\ \hline
% Indonesian       & 5702            \\ \hline
% Kiswahili        & 2755            \\ \hline
% Korean           & 1625            \\ \hline
% Russian          & 6490            \\ \hline
% Telugu           & 5563            \\ \hline
% \end{tabular}%
% }
% \caption{TydiQA No. of instances for all 9 languages of Gold Passage Task}
% \label{table:TydiQA_no_of_instances}
% \end{table}



\begin{table}[!h]
\centering
% \caption{TyDi QA No. of instances for all 9 languages of Gold Passage Task}
\label{table:TydiQA_no_of_instances}
\begin{tabular}[t]{lc}
\toprule
&Number of Instances \\
\midrule
Arabic           & 14805           \\ 
Bengali          & 2390            \\ 
English          & 3696            \\ 
Finnish          & 6855            \\ 
Indonesian       & 5702            \\ 
Kiswahili        & 2755            \\ 
Korean           & 1625            \\ 
Russian          & 6490            \\ 
Telugu           & 5563            \\
\bottomrule
\end{tabular}
\caption{TyDi QA No. of instances for all 9 languages of Gold Passage Task}
\end{table}%


\textbf{Monolingual - Few-shot Setting}

In the TyDi QA GoldP dataset, we have a total of 9 languages. For each of the experiments done in the monolingual few shot setting, we have selected one language at a time and added 10, 20 or 50 instances of that language from the training set of TyDi QA GoldP dataset to the SQuAD dataset and we have evaluated our trained model on the TyDi QA dev set for that corresponding language only.

\textbf{Multilingual - Few-shot Setting}

For the multilingual few shot setting, we have considered all of the languages and added 10, 20 or 50 TyDi QA training set instances from each of the languages to the SQuAD dataset and evaluated on the full TyDi QA dev dataset.

In both of the settings, we found that, the hypothesis is not rejected, it increased the performance compared to the zero shot baseline.

\subsection{Hypothesis 2 - Monolingual Full TyDi QA Setting}
In this hypothesis, we assumed that training/testing on every single language separately may tune the model more suitably for that specific language, and consequently gain better performance on that language. For training phase, we have separated the whole TyDi QA train set into subsets, each consisting of the instances from that specific language only. We also made separate TyDi QA dev sets for each of the languages and evaluated our trained model on these corresponding dev sets separately.

\subsection{Improvement Results - (SQuAD Few-shot)}
Table \ref{table:fullfewshotResults} shows the F1 scores for both of the few shot experiments mentioned in the previous section. Highlighted values indicate the higher F1 score compared to baseline Squad Zero Shot Setting. As expected, our few shot experiments has gained better F-1 scores than the zero shot baseline result. 

%\begin{table*}[!h]
%\caption{Full Few Shot Results} \label{table:fullfewshotResults}
%\centering  % not needed, since table is as wide as text block
%\begin{tabularx}{\textwidth}{@{}lYYYYYY@{}}
%\toprule
%&\multicolumn{3}{c}{\bfseries Monolingual Few Shot}
%&\multicolumn{3}{c}{\bfseries Multilingual Few Shot} \\
%\cmidrule(lr){2-4} \cmidrule(l){5-7} 
%&10 total instances + SQuAD 
%&20 total instances + SQuAD 
%&50 total instances + SQuAD 
%&10 per language (90 in total) + SQuAD 
%&20 per language (180 in total) + SQuAD
%&50 per language (450 in total) + SQuAD\\
%\midrule
%English & 73.74 & \textbf{74.69} & 73.92 & 73.28 & 74.47 & 72.98 \\
%Arabic & 64.75 & 63.51 & 64.89 & 63.42 & 64.55 & \textbf{70.76} \\
%Bengali & 62.83 & 60.53 & \textbf{66.45} & 62.63 & 64.74 & 61.36 \\
%Finnish & 68.21 & 66.62 & \textbf{70.90} & 68.10 & 69.42 & 70.16 \\
%Indonesian & 69.33 & 72.11 & 73.27 & 68.61 & 73.66 & \textbf{74.11} \\
%Kiswahili & 59.90 & 63.94 & 70.08 & 64.83 & 65.19 & \textbf{72.19} \\
%Korean  & 24.93 & 28.58 & 26.06 & 25.31 & \textbf{29.32} & 27.38 \\
%Russian & 65.56 & 66.78 & 66.30 & 65.64 & \textbf{66.97} & 66.28 \\
%Telugu & 50.70 & 63.04 & 62.53 & 47.46 & 62.68 & \textbf{68.24} \\
%Overall  & --     & --     &--  & 61.87 & 65.46 & \textbf{67.36} \\
%\bottomrule
%\end{tabularx}
%\end{table*}

\subsubsection{Analysis: Hypothesis 1 - Few-shot Setting}
In SQuAD zero shot setting, we can get an F1 score of 57.50 and just by adding 50 instances from each language in the few shot multilingual setting we can get an F1 score of 67.36. Here, we have added a total of 450 instances which is about 0.90\% of the TyDi QA train dataset. This is an indication that, we can get a moderately good performance with much fewer instances. In low resource settings, where getting training labels is much harder, this is significantly important. 

Some comparisons between few shot and zero shot results are depicted in Figure \ref{fig:tydiqa_few_zero_all} and \ref{fig:tydiqa_few_zero_all_individua}.
\begin{figure}[h!]
\centering
\includegraphics[scale=0.55, center]{Figures/FS-All-HQ-Serif.jpg}
\caption{TyDi QA GoldP task: Few Shot vs Zero-shot on all languages}
\label{fig:tydiqa_few_zero_all}
\end{figure}
\begin{figure}[h!]
\centering
\includegraphics[scale=0.55, center]{Figures/FS-indiv-HQ-Serif.jpg}
\caption{TyDi QA GoldP task: Few Shot vs Zero-shot on all/individual 9 languages}
\label{fig:tydiqa_few_zero_all_individua}
\end{figure}
It's not absolutely clear from our experiments whether multilingual or monolingual few shot is a better choice. In most cases, multilingual few shot experiments yielded better F1 scores. This is a reasonable fact as many languages has similarities among them.
% \begin{table}[H]
% \centering
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{p{2cm}| p{1.5cm}|p{1.5cm}|p{1.5cm}}
% \toprule
% Language & 90 TyDi   (10 per language) + SQuAD & 180 TyDi   (20 per language) + SQuAD & 450 TyDi (50 per language) + SQuAD \\ \midrule
% English    & 73.28 & \textbf{74.47} & 72.98 \\ 
% Arabic     & 63.42 & 64.55 & \textbf{70.76} \\ 
% Bengali    & 62.63 & \textbf{64.74} & 61.36 \\ 
% Finnish    & 68.10 & 69.42 & \textbf{70.16} \\ 
% Indonesian & 68.61 & 73.66 & \textbf{74.11} \\ 
% Kiswahili  & 64.83 & 65.19 & \textbf{72.19} \\ 
% Korean     & 25.31 & \textbf{29.32} & 27.38 \\ 
% Russian    & 65.64 & \textbf{66.97} & 66.28 \\ 
% Telugu     & 47.46 & 62.68 & \textbf{68.24} \\ \midrule
% Overall    & 61.87 & 65.46 & \textbf{67.36} \\ \bottomrule
% \end{tabular}%
% }
% \caption{Hypothesis 1 - Few-shot Setting.Highlights values  indicates the higher F1 score compared to baseline Squad Zero Shot Setting
% }
% \label{table:ImprovementResult_Hypothesis1}
% \end{table}

\an{How many times were these experiments run? Since we are randomly sampling 10 training instances per language, it is important to do these experiments many times with random sampling of the training data and report average and standard deviation across all runs. e.g. 5 or 10 runs, depending on how much times these take}

\navid{It was just once for each experiment. Will do that multiple times.}

\subsubsection{Analysis: Hypothesis 2 - Monolingual Setting}
In the monolingual setting, we have trained and evaluated on individual TyDi QA languages and for all of the languages we got worse results than when the model was trained and evaluated on all of the languages. For this reason, we can safely disregard this hypothesis. Many languages here have similarities in underlying structure and thus yields better performance when more instances even in different languages are added to the training set. So, a mere assumption about getting better performance when training and evaluating on a single language is incorrect.  

Table \ref{fig:hypothesis2} shows the results we obtained from our experiments. Highlighted values indicate the higher F1 score compared to monolingual Setting.

\begin{table}[!h]
\centering
% \caption{TyDi QA - Monolingual vs. All-in-once}
\label{fig:hypothesis2}
\begin{tabular}[t]{lcc}
\toprule
&Monolingual & All-in-once\\
\midrule
English    & 70.59 & \textbf{77.51} \\
Arabic     & 80.43 & \textbf{82.44} \\
Bengali    & 69.50 & \textbf{78.94} \\
Finnish    & 76.94 & \textbf{80.06} \\
Indonesian & 81.83 & \textbf{85.36} \\
Kiswahili  & 77.83 & \textbf{83.78} \\
Korean     & 27.67 & \textbf{34.55} \\
Russian    & 71.70 & \textbf{76.46} \\
Telugu     & 75.33 & \textbf{78.27} \\
Overall    & --     & 77.87 \\
\bottomrule
\end{tabular}
\caption{TyDi QA - Monolingual vs. All-in-once}
\end{table}%

% \begin{table}[H]
% \centering
% \noindent
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{|p{2cm}| p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% Language &
%   \begin{tabular}[c]{@{}c@{}}10 TyDi +\\(Mono) \\ SQuAD\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}20 TyDi +\\(Mono) \\ SQuAD \end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}50 TyDi +\\(Mono) \\ SQuAD\end{tabular} \\ \hline
% English    & 73.74 & \textbf{74.69} & 73.92 \\ \hline
% Arabic     & 64.75 & 63.51 & \textbf{64.89} \\ \hline
% Bengali    & 62.83 & 60.53 & \textbf{66.45} \\ \hline
% Finnish    & 68.21 & 66.62 & \textbf{70.90} \\ \hline
% Indonesian & 69.33 & 72.11 & \textbf{73.27} \\ \hline
% Kiswahili  & 59.90 & 63.94 & \textbf{70.08} \\ \hline
% Korean     & 24.93 & \textbf{28.58} & 26.06 \\ \hline
% Russian    & 65.56 & \textbf{66.78} & 66.30 \\ \hline
% Telugu     & 50.70 & \textbf{63.04} & 62.53 \\ \hline
% Overall    & -     & -     & -     \\ \hline
% \end{tabular}%
% }
% \caption{Hypothesis 2 - Monolingual Setting. Highlights values  indicates the higher F1 score compared to baseline Squad Zero Shot Setting
% }
% \label{table:ImprovementResult_Hypothesis2}
% \end{table}

%\begin{table}[H]
%\centering
%\small
%\resizebox{0.3\textwidth}{!}{%
%\begin{tabular}{|p{1.5cm}| p{1.5cm}|}
%\hline
%        TyDiQA \\ Languages & No. of instances \\ \hline
%        Arabic           & 14805           \\ \hline
%        Bengali          & 2390            \\ \hline
%        English          & 3696            \\ \hline
%        Finnish          & 6855            \\ \hline
%        Indonesian       & 5702            \\ \hline
%        Kiswahili        & 2755            \\ \hline
%        Korean           & 1625            \\ \hline
%        Russian          & 6490            \\ \hline
%       Telugu           & 5563            \\ \hline
%\end{tabular}%
%}
%\caption{TydiQA No. of instances for all 9 languages of Gold Passage Task}
%\label{table:TydiQA_no_of_instances}
%\end{table}

% \begin{table}[H]
% \small
% \centering
% \resizebox{0.45\textwidth}{!}{%
% \begin{tabular}{|p{1.75cm}| p{1.5cm}|p{1.5cm}|}
% \hline
% Language & Monolingual TyDi QA Train \& Test & \begin{tabular}[c]{@{}l@{}}\\ \\ \\ Training on \\ all  
% once,\\ Testing \\separately\end{tabular} \\ \hline
% English    & 70.59 & 77.51 \\ \hline 
% Arabic     & 80.43 & 82.44 \\ \hline
% Bengali    & 69.50 & 78.94 \\ \hline
% Finnish    & 76.94 & 80.06 \\ \hline
% Indonesian & 81.83 & 85.36 \\ \hline
% Kiswahili  & 77.83 & 83.78 \\ \hline
% Korean     & 27.67 & 34.55 \\ \hline
% Russian    & 71.70 & 76.46 \\ \hline
% Telugu     & 75.33 & 78.27 \\ \hline
% Overall    & -     & 77.87 \\ \hline
% \end{tabular}%
% }
% \caption{TydiQA Results: Monolingual vs. All in once }
% \label{tab:TydiQA_MonolingualvsAll}
% \end{table}



\subsection{Task 1: Train on all SQuAD Translated instances (all 9 languages) and evaluated on TyDiQA dev instances}


\begin{table}[!h]
\centering
% \caption{Task 1: Training on all SQuAD Translated instances ( all 9 languages) and evaluated on TyDiQA dev instances Results}
\label{table:All_Squad_Translated_instances}
\begin{tabular}[t]{lc}
\toprule
& \textbf{Multilingual Setting} \\
\midrule
English & 74.92  \\
Bengali & 58.38 \\
Finnish & 66.74 \\
Indonesian & 65.18  \\
Kiswahili & 69.37  \\
Korean  & 30.88  \\
Russian & 60.19  \\
Telugu & 44.68  \\
Overall & 73.59  \\
Overall without \\ English \& Korean & 61.42 \\
Overall without Korean & 63.11 \\
\bottomrule
\end{tabular}
\caption{Task 1: Training on all SQuAD Translated instances ( all 9 languages) and evaluated on TyDiQA dev instances Results}
\end{table}%

\subsection{Task 2 and 3a: Train on Squad + 50/100/200/500 unique instances from each of the google translated Squad langauges (8 langauges). (50/100/200/500)*8 unique qa pairs.}

\begin{table*}[!h]
\centering
% \caption{Task 2 and 3a: Train on Squad + 50/100/200/500 unique instances from each of the google translated Squad langauges (8 langauges). (50/100/200/500)*8 unique qa pairs.}
\label{table:task2}
\begin{tabular}[t]{lcccc}
\toprule
 & Squad+50 & Squad+100 & Squad+200 & Squad+500\\
\midrule
English & 73.77 & 72.45 & 74.43 & 73.65\\
Arabic & 64.02 & 62.25 & 62.71 & 63.25 \\
Bengali & 62.39 & 66.61 & 64.18 & 69.51\\
Finnish & 68.41 & 68.40 & 68.76 & 67.92\\
Indonesian & 69.68 & 68.63 & 70.75 & 70.88\\
Kiswahili & 59.72 & 64.86 & 66.08 & 69.77\\
Korean  & 28.68 & 29.93 & 30.25 & 30.52\\
Russian & 66.84 & 67.11 & 66.21 & 66.67\\
Telugu & 48.06 & 47.50 & 48.28 & 49.06\\
Overall & 62.73 & 63.62 & 63.85 & 65.30\\
\bottomrule
\end{tabular}
\caption{Task 2 and 3a: Train on Squad + 50/100/200/500 unique instances from each of the google translated Squad langauges (8 langauges). (50/100/200/500)*8 unique qa pairs.}
\end{table*}%


\subsection{Task 3B: TydiQA Monolingual \& Multilingual few-shot setting}


\begin{table*}[!h]
% \caption{Task 3B: Full Few Shot Results: TydiQA Monolingual \& Multilingual few-shot setting} \label{table:fullfewshotResults}
%\centering  % not needed, since table is as wide as text block
\begin{tabularx}{\textwidth}{@{}lYYYYYYYYY@{}} 
\toprule
&\multicolumn{3}{c}{\bfseries Monolingual  Few Shot}
&\multicolumn{6}{c}{\bfseries Multilingual Few Shot} \\
\cmidrule(lr){2-4} \cmidrule(l){5-10} 
&10 total instances + SQuAD 
&20 total instances + SQuAD 
&50 total instances + SQuAD 
&10 per language (90 in total) + SQuAD 
&20 per language (180 in total) + SQuAD
&50 per language (450 in total) + SQuAD
&100 per language (900 in total) + SQuAD 
&200 per language (1800 in total) + SQuAD
&500 per language (4500 in total) + SQuAD\\
\midrule
English & 73.74 & 74.69 & 73.92 & 73.70 & 74.47 & 73.46  & 74.21 & 73.95 & \textbf{76.13} \\
Arabic & 64.75 & 63.51 & 64.89 & 64.56 & 65.88 & 69.18  & 72.51 & 74.76 & \textbf{76.32} \\
Bengali & 62.83 & 60.53 & 66.45 & 62.92 & 66.85 & 65.80  & 70.86 & 70.49 & \textbf{74.50} \\
Finnish & 68.21 & 66.62 & 70.90 & 66.52 & 69.04 & 68.97  & 71.87 & 74.09 & \textbf{78.23} \\
Indonesian & 69.33 & 72.11 & 73.27 & 69.95 & 72.48 & 68.97  & 75.48 & 77.74 & \textbf{81.40} \\
Kiswahili & 59.90 & 63.94 & 70.08 & 63.09 & 64.17 & 68.75  & 72.29 & 76.45 & \textbf{79.20} \\
%Korean  & 24.93 & 28.58 & 26.06 & 25.31 & \textbf{29.32} & 27.38  & 73.28 & 74.47 & 72.98 \\
Russian & 65.56 & 66.78 & 66.30 & 65.94 & 66.93 & 67.17  & 69.27 & 69.79 & \textbf{73.32} \\
Telugu & 50.70 & 63.04 & 62.53 & 59.55 & 63.73 & 66.16  & 69.32 & 69.96 & \textbf{73.73} \\
Overall (Avg w/o Eng)  & --     & --     &--  & 64.64 & 67.01 & 67.86  & 71.65 & 73.33 & \textbf{76.67} \\
\bottomrule
\end{tabularx}
\caption{Task 3B: Full Few Shot Results: TydiQA Monolingual \& Multilingual few-shot setting}
\end{table*}


\subsection{Task 3C: Trained on English SQuAD plus all SQuAD translations, fine-tuned on 500 random instances from TyDiQA train set per language (9*500 in total), evaluated on TyDiQA dev set}

\begin{table}[!h]
\centering
% \label{fig:hypothesis2}
\begin{tabular}[t]{lccc}
\toprule
&mBERT & XLMR-L & Baseline\\
\midrule
% English    & \textbf{77.87} & 73.21 & 76.8 \\
Arabic     & 78.81 & 72.82 & \textbf{81.7} \\
Bengali    & \textbf{80.02} & 78.28 & 75.4 \\
Finnish    & \textbf{79.48} & 78.54 & 79.4 \\
Indonesian & 82.78 & 84.73 & \textbf{84.8} \\
Kiswahili  & \textbf{83.63} & 80.29 & 81.9 \\
% Korean     & 31.86 & 36.20 & \textbf{69.2} \\
Russian    & 72.50 & 74.95 & \textbf{76.2} \\
Telugu     & 73.49 & 78.11 & \textbf{83.3} \\
Average    & 78.67 & 78.24 & \textbf{80.4} \\
SD         & 3.94  & 3.51  & 3.28 \\
\bottomrule
\end{tabular}
\caption{Task 3C - Fixed budget allocation (500 per language, 4500 in total) vs. TyDi QA Baseline}
\end{table}%


\subsection{Task 3C.1: disproportional TyDiQA budget allocation, trained on English SQuAD plus all SQuAD translations, fine-tuned on 4500 random instances from TyDiQA train set per language (if available, otherwise maximum available TyDiQA train set), evaluated on TyDiQA dev set}


\begin{table*}[!h]
\centering
% \caption{Task 3C.1 \& 3C.2 - Disproportional Allocation}
% \label{fig:hypothesis2}
\begin{tabular}[t]{lcccccccc}
\toprule
&Arabic & Bengali* & Finnish & Indonesian & Russian & Kiswahili* & Telugu & 3C \\
\midrule
Arabic    & \textbf{81.76} & 66.32 & 75.47 & 76.74 & 74.48 & 72.46 & 70.65 & 78.81 \\
Bengali   & 61.99 & 77.71 & 72.64 & 67.41 & 66.71 & 67.08 & 70.16 & \textbf{80.02}  \\
Finnish   & 77.57 & 71.54 & \textbf{79.68} & 76.94 & 76.27 & 75.00 & 73.64 & 79.48  \\
Indonesian  & 79.23 & 72.81 & 80.96 & \textbf{83.92} & 80.99 & 77.39 & 73.71 & 82.78 \\
Russian   & 68.03 & 66.50 & 70.62 & 70.25 & \textbf{75.72} & 66.42 & 68.11 & 72.50  \\
Kiswahili  & 72.76 & 78.10 & 78.48 & 77.28 & 78.81 & \textbf{84.02} &  77.10 & 83.63 \\
Telugu    & 50.50 & 51.96 & 52.22 & 52.18 & 69.36 & 74.97 & \textbf{78.19} &  73.49 \\
Average   & 70.26  & 69.28 & 72.87 & 72.10 & 74.62 & 73.91 & 73.08 & \textbf{78.67}  \\
SD   &  10.25 & 8.30 & 9.11 & 9.51 & 4.66 & 5.62 & 3.42 & 3.94 \\
\bottomrule
\end{tabular}
\caption{Task 3C-1: Disproportional Allocation with minimum(available budget, 4500) for each language}
\end{table*}%

\subsection{Task 3C-2: disproportional TyDiQA budget allocation for 3 randomly picked languages, trained on English SQuAD plus all SQuAD translations, fine-tuned on 4500 random instances from TyDiQA train set (1500 per for each 3 language), evaluated on TyDiQA dev set}

\begin{table*}[!h]
\centering

\begin{tabular}[t]{lcccccccc}
\toprule
                 & ben-rus-tel & tel-ind-swa & fin-rus-swa    & ara-rus-tel & ara-rus-fin & swa-ind-fin & ara-ind-swa & 3C  \\
\midrule
English          & 75.80       &  76.11      & \textbf{78.49}         & 75.73       &  76.52      &  76.11      &  78.28      & 77.87 \\
Arabic           & 72.16       & 75.68       &  76.37         & 79.31       & \textbf{80.50}      &  77.17      & 79.52      & 78.81 \\ 
Bengali          & 79.00       &  65.46      &  66.35         & 66.79       &  68.89      &  68.51      &  65.44      & \textbf{80.02} \\ 
Finnish          & 75.63       &  76.72      &  79.63          & 77.95       &  79.18      &  \textbf{79.72}      &  76.85      & 79.48 \\ 
Indonesian       & 74.82       & 83.23       &  80.32        & 79.27       &  80.65      &  \textbf{84.23}      &  83.88      & 82.78 \\ 
Kiswahili        & 77.10       &  84.65      &  \textbf{84.79}& 79.92       &  77.51      &  83.00      &  83.55      & 83.63 \\ 
Russian          & 74.45       &  71.16      &  \textbf{74.86}& 74.35       &  74.34      &  71.23      &  68.89      & 72.50 \\ 
Telugu           & 76.75       &\textbf{77.20}&  53.39        & 76.97       &  53.61      &  51.47      &  50.60      & 73.49 \\
Average          & 75.70       &  76.30      &  73.67         & 76.36       &  73.53      &  73.62      &  72.67      &\textbf{78.67} \\
SD               & 2.02        &  6.12       &  9.83          & 4.28        &  8.99       &  10.50      &  11.09      & 3.94   \\
\bottomrule
\end{tabular}
\caption{Task 3C-2: Disproportional Random 3}
\end{table*}%

% \begin{table}[!h]
% \centering
% \caption{Task 3C-2: Disproportional Random 3 Languages}
% \label{table:TydiQA_no_of_instances}
% \begin{tabular}[t]{lc}
% \toprule
% & Task 3C + translated XQuAD \\
% \midrule
% Arabic           & 74.15 \\ 
% Bengali          & 72.37 \\ 
% English          & 74.64 \\ 
% Finnish          & 75.99 \\ 
% Indonesian       & 75.74 \\ 
% Kiswahili        & 78.96 \\ 
% Korean           & 34.36 \\ 
% Russian          & 70.01 \\ 
% Telugu           & 73.53 \\
% Overall          & 72.17 \\
% Overall (Avg)    &       \\
% \bottomrule
% \end{tabular}
% \end{table}%



% \begin{table*}[!h]
% \caption{Task 3C.1 - Disproportional Allocation} \label{table:fullfewshotResults}
% %\centering  % not needed, since table is as wide as text block
% \begin{tabularx}{\textwidth}{@{}lYYYYYY@{}}
% \toprule
% &\multicolumn{3}{c}{\bfseries Monolingual Few Shot}
% &\multicolumn{3}{c}{\bfseries Multilingual Few Shot} \\
% \cmidrule(lr){2-4} \cmidrule(l){5-7} 
% &10 total instances + SQuAD 
% &20 total instances + SQuAD 
% &50 total instances + SQuAD 
% &10 per language (90 in total) + SQuAD 
% &20 per language (180 in total) + SQuAD
% &50 per language (450 in total) + SQuAD\\
% \midrule
% English & 73.74 & \textbf{74.69} & 73.92 & 73.28 & 74.47 & 72.98 \\
% Arabic & 64.75 & 63.51 & 64.89 & 63.42 & 64.55 & \textbf{70.76} \\
% Bengali & 62.83 & 60.53 & \textbf{66.45} & 62.63 & 64.74 & 61.36 \\
% Finnish & 68.21 & 66.62 & \textbf{70.90} & 68.10 & 69.42 & 70.16 \\
% Indonesian & 69.33 & 72.11 & 73.27 & 68.61 & 73.66 & \textbf{74.11} \\
% Kiswahili & 59.90 & 63.94 & 70.08 & 64.83 & 65.19 & \textbf{72.19} \\
% Korean  & 24.93 & 28.58 & 26.06 & 25.31 & \textbf{29.32} & 27.38 \\
% Russian & 65.56 & 66.78 & 66.30 & 65.64 & \textbf{66.97} & 66.28 \\
% Telugu & 50.70 & 63.04 & 62.53 & 47.46 & 62.68 & \textbf{68.24} \\
% Overall  & --     & --     &--  & 61.87 & 65.46 & \textbf{67.36} \\
% \bottomrule
% \end{tabularx}
% \end{table*}


\subsection{Task 4A: Modify English SQuAD Dataset by keeping the language of context and answers fixed (English) and changing the language of the questions using different languages (except English)
}

\subsection{Task 4B: Modify English SQuAD Dataset by changing both context and answers to same language (except English) and changing the language of the questions using different languages. 
}



\begin{table*}[!h]
%\centering  % not needed, since table is as wide as text block
\begin{tabularx}{\textwidth}{@{}lYYYYYY@{}} %YYY
\toprule

&\multicolumn{3}{c}{\bfseries Change language of Question only }
&\multicolumn{3}{c}{\bfseries Change all; Context \& answers the same} \\

\cmidrule(lr){2-4} \cmidrule(l){5-7} 

& Modified Squad 
& Squad + Modified Squad 
& Modified Squad + 500 instances 
& Modified Squad 
& Squad + Modified Squad 
& Modified Squad + 500 instances \\
\midrule
%English & 75.06 & 0 & 73.49 & 0  \\
Arabic & 62.17 & 65.62 & 77.96 & 60.51 & 65.98 & 78.70  \\
Bengali & 67.33 & 68.55 & 76.16 & 58.60 & 62.44 & 75.00  \\
Finnish & 67.42& 71.67 & 79.51 & 62.98 & 67.58 & 78.55   \\
Indonesian & 66.45 & 70.33 & 84.10 & 61.89 & 66.44 & 83.46 \\
Kiswahili & 70.32 & 75.48 & 80.01 & 62.66 & 68.55 & 82.51  \\
Russian & 64.71 & 66.16 & 73.28 & 61.01 &  65.64 & 73.16  \\
Telugu & 48.32 & 49.36 & 74.95 & 43.62 & 51.81 & 75.28  \\
%Overall  & 64.90     & 0     &63.23  & 0 \\
Avg & 63.82 & 66.74 & \textbf{78.00} & 58.76 & 64.07 & \textbf{78.09} \\
SD & 6.74 & 7.75 & 3.35 & 6.33 & 5.31 & 3.60 \\
\bottomrule
\end{tabularx}
\caption{Task 4A and 4B} \label{table:fullfewshotResults}
\end{table*}








\subsection{Task 5: Squad + All Squad translations, fine-tuned on 500 instances from each of the TyDiQA train languages, fine tuned on All XQuAD translation}

\begin{table}[!h]
\centering

\label{table:TydiQA_no_of_instances}
\begin{tabular}[t]{lc}
\toprule
& Task 3C + translated XQuAD \\
\midrule
Arabic           & 74.15 \\ 
Bengali          & 72.37 \\ 
% English          & 74.64 \\ 
Finnish          & 75.99 \\ 
Indonesian       & 75.74 \\ 
Kiswahili        & 78.96 \\ 
% Korean           & 34.36 \\ 
Russian          & 70.01 \\ 
Telugu           & 73.53 \\
% Overall          & 72.17 \\
Average          &  74.39  \\
SD               &  2.65  \\
\bottomrule
\end{tabular}
\caption{Task 5}
\end{table}%

==> Conclusion.tex <==
\section{Conclusion}
%The  multilingual  dataset  is  an  expensive/cumbersome  procedure.Therefore,any  data-efficient  approach  which  are  would be  able  to  increase  the  performance  of  the model  to  some  extend  only  using  a  limited amount  of  augmented data  would  be  lucrative.In  this  project,  we’ve  been  focusing on one of the state-of-the-art multilingual QA benchmarks, known as TyDi QA (Clark et al.,2020) and carried out our experiments in two phases:   (1)  reproducing  the  baseline gold-passage results using pre-trained multilingual-BERT (Huggingface - mBERT), and (2) improving the SQuAD (Rajpurkar et al., 2016b)zero-shot  performance  by  utilizing  a  limited portion of the TyDi QA training set and introducing the few-shot setting.
To sum up, we started with TyDi QA (which is one of the most recent multilingual QA benchmarks) and carried out our experiments in two phases. First, we reproduced the baseline results using pre-trained \cite{huggingface:mBERT} and even achieved slightly higher F-1 score, compared to the original baseline \cite{clark2020tydi} in most of the individual languages, but slightly lower F-1 score has been achieved in overall (i.e. full training and testing on all languages). Afterwards, we augmented the existing, monolingual SQuAD \cite{rajpurkar2016squad} with a relatively small portion of the TyDi QA train set, improved the SQuAD Zero-shot setting and introduced it as Few-shot setting. Talking about failures, we failed to reproduce the baseline and improved results for Korean language (that we need to work on in the future). Also, we are planning to expand the analysis of finding the optimum trade-off (i.e. the best value of the number of instances to be added to SQuAD in order to achieve the highest performance while utilizing the least possible amount of resources) for the Few-shot setting. Moreover, we aim for exploiting the power of Neural Machine Translation (NMT) to go further on making our model more data-efficient by training on the original instances and test on the translated version of the instances. If this hypothesis works in practice, we can generate a synthetic multilingual QA dataset, only using the existing monolingual (English only) datasets like SQuAD \cite{rajpurkar2016squad}.

\ifaclfinal
\section{Acknowledgments}
 
ARGO, the research computing cluster provided by the Office of Research Computing at George Mason University supported us in running the majority of computations.
\fi


==> experiments.tex <==
\section{Experiments}
\subsection{Monolingual Experiments}
\subsubsection{Monolingual}
In the monolingual setting, at each training phase, we trained only on one individual TyDiQA language and evaluated on the corresponding TyDiQA dev set language. 

The purpose of this experiment was to understand how individual languages contribute to the QA problem. More specifically, we wanted to know whether training on monolingual settings give better performance scores or a multilingual model does because of more data availability and similarities among languages.

For all of the languages, we got worse results than when the model was trained and evaluated on all of the languages (Table \ref{fig:hypothesis2}). Many  languages  here have similarities in underlying structure and thus yields  better  performance  when  more  instances even in different languages are added to the training set.

\subsubsection{Monolingual Few Shot}
We have selected one language at a time and added 10, 20 or 50 instances of that language from the training set of TyDiQA GoldP dataset to the Squad dataset and  evaluated our trained model on the TyDiQA dev set for that corresponding language only.

The purpose of this experiment was to compare the results with multilingual few shot setting (Table \ref{table:fullfewshotResults} which is described later. 

Even though, monolingual setting with all the instances described at the beginning of this section clearly performed worse than multilingual setting, the few shot monolingual experiments showed very similar if not better F1 scores than the respective multilingual experiments. 

\subsection{Multilingual Experiments}
In all the multilingual experiments, we have added instances from different languages either from translated Squad/Xquad instances, or from TyDiQA train languages.

\subsubsection{Multilingual Few Shot}
For the multilingual few shot setting, we have considered all of the languages and added 10, 20 or 50 TyDi QA training set instances from each of the languages to the SQuAD dataset and evaluated on the full TyDi QA dev dataset.

The objective of this few shot experiment was to gain insights on how little amount of data we can use to get similar results to the baseline scores.

From our results (Table \ref{table:fullfewshotResults}), we can see that by adding 500 instances from every language which is a total of about 9\% of the whole TyDiQA train dataset, we get an F1 score of 76.67 which is close to our reproduced baseline score of 80.76.

\subsubsection{Translation}
In the next set of experiments we have used google translator API to translate the Squad or Xquad instances to the 8 languages (except English). Detail about our translation process is described in the Appendix.

\textbf{Translation - Few Shot}
These experiments are similar to the multilingual few shot experiments, the only difference is that instead of augmenting the Squad dataset with instances from TyDiQA train languages, we use instances from the translated Squad dataset. 

The purpose of this experiment was to see if the expensive labelling effort can be bypassed with automated translations of existing datasets.

We have seen that using all of the Squad translations yield worse performance than using some translated instances. (\ref{table:All_Squad_Translated_instances} & \ref{table:task2}). It also turns out that, augmenting Squad with as small as 20 instances yields better performance than the highest we got from using 500 translated instances (\ref{table:task2}).

\textbf{Translation-Few shot and Fine tuning on TyDiQA}



==> literature_review.tex <==
\section{Literature Review}
\label{section:literaturereview}

\input{monolingual_qa.tex}
\input{multilingual_qa.tex}
\input{baseline.tex}



==> monolingual_qa.tex <==
\subsection{Mono-lingual QA Benchmarks}
% \subsubsection{TriviaQA} Question answering also can be interpreted as an activity in validating the knowledge of experts by finding the answer to trivia questions that are carefully arranged by someone who already knows the answer  with the end goal that precisely one answer is correct like TriviaQA \cite{clark2020tydi}. The goal of reading comprehension (RC) systems to answer any question that may be presented against the facts in some reference text is challenging due to some reasons including questions having highly compositional semantics, finding the proper answer can require complex reasoning and individual facts are often difficult to pass through text due to lexical and syntactic variation.
% TriviaQA is meant to simultaneously test all of those challenges. TriviaQA integrates 95K question-answer pairs authored by trivia enthusiasts and independently gathered evidence documents, six for each question overall, that provide prime quality far off supervision to respond to the answering the questions. TriviaQA has some finer properties including relatively complex and compositional questions, a significant amount of syntactic and lexical variability between questions and corresponding answer-evidence sentences, and requirement of more cross sentence reasoning to explore answers. TriviaQA also proposed two baseline algorithms. One is a feature-based classifier and the other is a state-of-the-art neural network that performs comparatively well on SQuAD reading comprehension \cite{DBLP:journals/corr/JoshiCWZ17}. However, Neither methodology draws close to human performance (performance 80), recommending that TriviaQA might be a difficult testbed that is worth noteworthy future study.
% \subsubsection{NewsQA} NewsQA \cite{trischler2016newsqa} is a machine comprehensive (MC) dataset comprising 119,633 human-generated QA pairs on a set of 12,744 news articles from CNN. There are other machine comprehensive datasets which lack in quality and quantity because of small human generated training data or large synthetic data comprising questions which are not natural. NewsQA was created while keeping in mind these shortcomings and it poses a more challenging MC task. 
% Some of the key characteristics of this dataset are as follows.
% Answers are not single words rather a span of words.
% Some question doesn’t have any answer from the article
% No candidate answers to choose from
% The dataset was created such that there are lexical and syntactic divergence between QA.
% It’s a challenging dataset in the sense that the answers to the questions require a deep reasoning which is beyond simple context or word matching.
% The baseline model for NewsQA is the match-LSTM model \cite{wang2016machine}. 
% As the match-LSTM network is computationally intensive, a faster lightweight model (BARB) was proposed by the authors. This model has the following 4 stages - GloVe \cite{pennington2014glove} word embedding generation, generating annotation matrix, feeding them to RNN and finally using CNN to predict the boundary span of the answer.


Stanford Question Answering Dataset (SQuAD) is the one the well-know English QA dataset 
% =====================================================================================
% Previous version:

% \subsubsection{SQuAD} Towards the ultimate objective of regular language understanding, the Stanford Question Answering Dataset (SQuAD) is a huge perusing cognizance dataset comprising 100,000+ various scope of questions presented by crowd workers on 500+ Wikipedia articles with publicly supported inquiry answer sets. \cite{DBLP:journals/corr/RajpurkarZLL16}. 

% In distinction to previous datasets, rather than providing a list of answer choices for every question, in SQuAD, the answer to each question is arranged as a segment of span or text, obtained from the corresponding reading passage, or even the question may well be unanswerable. The overall performance of their logistic regression model is highly satisfactory with 51.0 F1, against the human F1 of 86.8. Which has opened the door for plentiful development \cite{DBLP:journals/corr/RajpurkarZLL16}. The SQuAD dataset is unreservedly accessible to support the investigation of more expressive models. Existing datasets either center only around questions that are directly answerable, or utilize automatically generated unanswerable questions that are anything but difficult to identify. To address these weaknesses, the newest version of SQuAD combines existing SQuAD data with over 50,000 unanswerable questions. These are written adversarially by crowd workers to seem just like answerable ones. This latest version of SQuAD (SQuAD 2.0) systems forces models to understand when a question cannot be answered given the context \cite{DBLP:journals/corr/abs-1806-03822}. However, human performance (86.8) is much higher, showing that the SQuad dataset presents a decent challenge for future exploration. A strong neural system that gets 86 F1 on SQuAD 1.1 achieves only 66 F1 on SQuAD 2.0 indicating that this latest version of SQuAD is a challenging natural language understanding task for existing models.
% =====================================================================================

==> multilingual_qa.tex <==
\subsection{Multi-lingual QA Benchmarks}

% \subsubsection{MLQA} MLQA is a benchmark in SQuAD format for Multilingual QA containing question-answer pair instances in 7 different languages as: 12k in English, 5k in Arabic, 5k in German, 5k in Spanish, 5k in Hindi, 5k in Vietnamese and 5k in Chinese. 

% \textbf{MLQA annotation pipeline}: During the annotation process, a paragraph of English language and the target language is being selected in parallel. Then, each of the paragraphs is being divided into the sentence b and context around, named c. After that, the question and answer in both English and target language, along with their annotated answers are being generated by the human annotator.

%\subsubsection{MKQA} MKQA is an open-domain question answering which covers 26 diverse languages (14 language family branches) and comprises 10k question-answer pairs for each language which forms 260k question-answer pairs in total. Due to the wide range of languages this benchmark covers, MKQA has become a challenging dataset for question answering models to perform on low-resource languages, compared to the other benchmarks. In terms of comparison, XQA \cite{liu2019xqa}, MLQA \cite{conneau2019unsupervised}, XQuAD \cite{artetxe2019cross} and TyDiQA \cite{clark2020tydi} cover 28k pairs over 9 languages, 46k pairs over 7 languages, 13k pairs over 11 languages, and 204k pairs over 11 languages respectively.

% \textbf{Dataset and Annotations:} MKQA has been generated by randomly sampling 10k realistic queries in English from Natural Questions dataset \cite{kwiatkowski2019natural} and translating them to 25 other languages by human annotators and increasing the quality and relevancy of the answer annotations. 


%%%%To be more specific, the human annotators/graders provide an Answer Type for each answer as Atomic value (like dates, numbers, ranges), Entities (Wikidata QIDs like people, locations, objects), Yes/No, Short answer, Long answer, and Unanswerable. Also, for each question, they’ve collected 5 answers, which has been normalized and admitted by at least 2 human annotators to be finalized.%
%Therefore, for each question-answer pair in English, there are question-answer pairs translated in 25 additional supported languages to incorporate linguistic diversity.

%\textbf{Task definition}: Given a question q in language l, the major task is to generate an answer prediction as one of the following types: (1) No answer, (2) Yes, (3) No, (4) Text Answer, in which “Text Answer” is a span of tokens (usually the start and end indices of the characters in the passage which contains the correct answer in the minimalistic manner).

%\textbf{Baseline models, experiments, and results:} Three different baseline models have been introduced for this benchmark: (1) M-BERT (Multilingual BERT pre-trained on Masked Language Modeling on 104 languages with 12 layers) \cite{clark2020tydi} (2) XLM (Cross-Lingual Model pre-trained on Masked Language Modeling and Translation Language Modeling on 100 languages with 16 layers) \cite{lample2019cross} and (3) XLM-R (an extension of XLM with RoBERTa architecture pre-trained on 100 languages with 24 layers) \cite{conneau2019unsupervised}. These baselines are evaluated on three different experiments of MQKA known as: (1) Zero Shot, (2)  Translate Test, and (3) Translate Train. In Zero Shot, each model is just fine-tuned on the Natural Question dataset and both questions and passages are in English during the training. During the test phase, each model is tested with questions in target language and passages in English, all from MKQA. In the Translate Test, each model is fine-tuned on Natural Questions in English during the training, but for the test phase, MKQA questions are translated from other languages into English, but the passages are in English all the time. In the Translate Train, during the training phase, models are trained on the questions which are translated into target languages from English, but during the test phase, models are given the queries in target language. However all the passages are in English in both training and testing phases. Finally, the XLM-R model outperforms the other two baselines in all three types of experiments in terms of Mean Bert F1 score (Zero-Shot = 45.4; Translate-Test = 42.9; Translate-Train = 46). In addition, Translate-Train yields the best results. Finally, the results show that there is enough room for improvement in MKQA.

\subsubsection{TyDi QA} TyDi QA is a multilingual question answering dataset which covers 11 typologically diverse languages and comprises 204K question-answer pairs. The languages of TyDi QA are diversified in steps with their typology which is the set of linguistic features expressed by each language in the simplest way such that the models perform well on this set to generalize across a high number of the world’s languages \cite{clark2020tydi}.

Passage Selection Task:

Minimal Answer Span Task:

Gold Passage (Gold-P) Task:

% Previous version: 

% \subsubsection{TyDi QA} Multilingual Models are a kind of Machine Learning model that can comprehend different languages. These multilingual modeling systems need challenging, trustworthy evaluations confidently to make more progress. TyDi QA is a multilingual question answering dataset which covers 11 typologically diverse languages and comprises 204K question-answer pairs. The languages of TyDi QA are diversified in steps with their typology which is the set of linguistic features expressed by each language in the simplest way such that the models perform well on this set to generalize across a high number of the world’s languages \cite{clark2020tydi}.

% \textbf{Task definition:} Given a multilingual model M provided by TyDi QA with a question q, as well as the content of a Wikipedia article, and request, the key tasks are to form two types of predictions:

% \textbf{Passage Selection Task:}  Given a list k of the Passages in the article. We have to do the following: Return (a) the index i of the passage p that answers the question or (b) NULL if it does not exist.\cite{clark2020tydi}

% \textbf{Minimal Answer Span Task:} Given an article having the full text. We have to do one in all following types: Return one of (a) some span of bytes in the article which contains the beginning b and end e byte indices of the minimal span which contain the complete and correct answers of the question; (b) YES or NO if the type of the question requires a yes/no answer so that it can extract a conclusion from the passage; (c) NULL if it is infeasible to generate a minimal answer for this question as many questions have no answers. \cite{clark2020tydi}

% \textbf{Simplified Gold Passage (GOLDP) Task:} Gold Passage (GOLDP) task is the simplified version of Minimal Answer Span Task, where instead of full Wikipedia document,the guaranteed the gold answer passage is provided. GOLDP task is more comparable to existing reading comprehension datasets like SQuAD, XQuAD, and MLQA. Thai and Japanese are eliminated due to the lack of whitespace breaks since the QA models are mostly designed to return the minimum span of the answer which consists of start and end indices. Therefore, for the languages without spaces in between the words (like Thai and Japanese), this structure cannot be used. So, either those languages should be removed or the structure of the system should be changed. 

% Thai and Japanese are eliminated due to the lack of whitespace breaks certain existing tools.

% Previous version: 
% A quantitative analysis for the quality of the data  and example-level qualitative linguistic analyses of observed language phenomena has been provided by TYDI QA that might not be found in English-only corpora. To produce a realistic information-seeking task and avoid priming effects, questions are written by folks who want to grasp the answer, but don’t know the answer yet, and therefore the data is collected directly in each language without the employment of translation. Quality on the primary tasks like Passage Selection (SELECTP) and Minimal Answer Span (MINSPAN) on TYDI QA  is provided by using 3 baselines - (1) a human predictor, (2) a naive first-passage baseline to predict the first passage assuming that most important facts are often summarized in the first paragraph of a Wikipedia article. And (3) the open-source most recently released multilingual BERT mBERT (Multilingual BERT pre-trained on Masked Language Modeling on 104 languages with 12 layers) \cite{devlin-etal-2019-bert} has been used here during a setup  similar as \cite{alberti2019bert}, during which all languages are trained jointly in a very single model. Over four fine-tuning replicas, precision, F1 and recall measurements are averaged for mBERT.

% Due to the computational limitation of finding a very large pool of annotators for 11 languages, a more pessimistic estimate of human performance has been considered. As a prediction, one human annotation is used and evaluated against the other two annotations. One is using bootstrap resampling to repeat this procedure for all the possible combinations of single vs. double annotators which correspond to the human evaluation methodology for SQuAD with the addition of bootstrapping to cut back variance. The estimate of human performance degraded where the  annotators disagreed which can cause an underestimate of human performance due to the fact that actually multiple answers may well be correct. Although at first glance, these F1 scores seemed low compared to simpler tasks like SQuAD, but yet a single human prediction on the Natural Questions short answer task (similar to the TYDI QA minimal answer task), scores only 57 F1 even with the advantage of evaluating against five annotations instead of just two and training on 30X more English training data.

\subsubsection{XQuAD} Artetxe et al. \cite{artetxe2019cross} has released a new benchmark for cross-lingual QA called XQuAD consisting of 240 paragraphs and 1190 question answer pairs from SQuAD v 1.1 \cite{rajpurkar2016squad}. Question answer and paragraphs are translated into ten languages by professional human translators. While TyDi QA allows answers to be None, meaning not extractable from the article, XQuAD model is always trained with a passage containing the answer. 

% Previous version: 
% \subsubsection{XQuAD} Artetxe et al. \cite{artetxe2019cross} has released a new benchmark for cross-lingual QA called XQuAD consisting of 240 paragraphs and 1190 question answer pairs from SQuAD v 1.1 \cite{rajpurkar2016squad}. Question answer and paragraphs are translated into ten languages by professional human translators. While TyDi QA allows answers to be None, meaning not extractable from the article, XQuAD model is always trained with a passage containing the answer. 

% \textbf{Proposed method:} This model is similar to m-BERT with some differences. XQuAD doesn’t have a shared vocabulary and it’s not trained jointly across multiple languages. 
% First, a monolingual BERT model is trained with MLM (masked language modeling) and NSP (next sentence prediction) objective in a language. 
% Secondly, this model is transferred to a new language. Here, the transformer parameters are frozen. This model is trained with the same objective as in the previous step to learn new token embeddings in this language.
% Now, the model is finetuned in the first language. In this stage, the token embeddings are frozen.
% Finally, the model is again transferred to the second language while using the learned token embeddings in step 2.

==> related_works.tex <==
\section{Related Work}
\label{section:relatedworks}

\an{This section is missing a lot of related work on few-shot learning for NLP. If there's any work that does few-shot experiments}

 Stanford Question Answering Dataset \textbf{SQuAD} is of the most well-known, huge perusing cognizance English QA dataset comprising 100,000+ various scope of questions presented by crowd workers on 500+ Wikipedia articles with publicly supported inquiry answer sets. \cite{DBLP:journals/corr/RajpurkarZLL16}. On the other hand, XQuAD dataset released by  Artetxe et al. \cite{artetxe2019cross} is cross-lingual one where Question answer and paragraphs are translated into ten languages by professional human translators. Recently released \textbf{TyDi QA} multilingual question answering dataset covers 11 typologically diverse languages and comprises 204K question-answer pairs. The languages of TyDi QA are diversified in steps with their typology which is the set of linguistic features expressed by each language in the simplest way such that the models perform well on this set to generalize across a high number of the world’s languages \cite{clark2020tydi}. %While TyDi QA allows answers to be None, meaning not extractable from the article, XQuAD model is always trained with a passage containing the answer.


Few shot setting is important when we need to evaluate how pre-trained models work based on a small amount of labeled data is available for fine-tuning. Existing research such as \cite{ram2021fewshot} has explored different few-shot setting having a sampling subsets of examples from bigger datasets. Their results indicated that careful design of pre-training schemes for span selection and model architecture is promising for the performance in the
few-shot settings even in a low-data scenario.
  

%Our findings indicate that careful design of pre-training schemes for span selection and model architecture can
%have a dramatic effect on performance in the
%few-shot settings even in a hundred examples scenario.


%In this work we explore the few-shot setting of extractive question answering, and demonstrate thatexisting methods, based on fine-tuning large pretrained language models, fail in this setup. We propose a new pretraining scheme and architecture for span selection that lead to dramatic improvements, reaching decent results even when only an order of a hundred examples are available. Our work shows that choices that are often deemed unimportant when enough data is available, again become crucial in the few-shot setting, opening the door to new methods that take advantage of prior knowledge on the downstream task during model development.




%\textbf{SQuAD} Stanford Question Answering Dataset (SQuAD) is of the most well-known English QA dataset which is a huge perusing cognizance dataset comprising 100,000+ various scope of questions presented by crowd workers on 500+ Wikipedia articles with publicly supported inquiry answer sets. \cite{DBLP:journals/corr/RajpurkarZLL16}. 

%\textbf{XQuAD}: Artetxe et al. \cite{artetxe2019cross} has released a new benchmark for cross-lingual QA called XQuAD consisting of 240 paragraphs and 1190 question answer pairs from SQuAD v 1.1 \cite{rajpurkar2016squad}. Question answer and paragraphs are translated into ten languages by professional human translators. While TyDi QA allows answers to be None, meaning not extractable from the article, XQuAD model is always trained with a passage containing the answer. 

%\textbf{TyDi QA} is a multilingual question answering dataset which covers 11 typologically diverse languages and comprises 204K question-answer pairs. The languages of TyDi QA are diversified in steps with their typology which is the set of linguistic features expressed by each language in the simplest way such that the models perform well on this set to generalize across a high number of the world’s languages \cite{clark2020tydi}.

\textbf{ I did not understand following:
Passage Selection Task:
Minimal Answer Span Task:
Gold Passage (Gold-P) Task:}
